Comparison Visual Instruction Tuning

Comparing two images in terms of Commonalities and Differences (CaD) is a fundamental human capability that forms the basis of advanced visual reasoning and interpretation. It is essential for the generation of detailed and contextually relevant descriptions, performing comparative analysis, novelty detection, and making informed decisions based on visual data. However, surprisingly, little attention has been given to these fundamental concepts in the best current mimic of human visual intelligence - Large Multimodal Models (LMMs). We develop and contribute a new two-phase approach CaD-VI for collecting synthetic visual instructions, together with an instruction-following dataset CaD-Inst containing 349K image pairs with CaD instructions collected using CaD-VI. Our approach significantly improves the CaD spotting capabilities in LMMs, advancing the SOTA on a diverse set of related tasks by up to 17.5%. It is also complementary to existing difference-only instruction datasets, allowing automatic targeted refinement of those resources increasing their effectiveness for CaD tuning by up to 10%. Additionally, we propose an evaluation benchmark with 7.5K open-ended QAs to assess the CaD understanding abilities of LMMs.

==> fig_tex/character_stats_instruction_template.tex <==

\begin{figure*}[ht]
\includegraphics[width=\columnwidth]{figures/fig_3.pdf}
\caption{
\label{fig:character_stats_instruction_template}
(a) Statistics of CaD characteristics (b) Instruction template    
}
\end{figure*}


==> fig_tex/word_distribution.tex <==


\begin{figure*}[ht]
\includegraphics[width=0.9\columnwidth]{figures/text_distribution.pdf}
\caption{
\label{fig:word_distribution}
(a) Distribution of characteristics (first two words) in the CaD summary collected in \OurDataPhaseOne (b) Distribution of question types (first five words) in the evaluation benchmark \OurBenchmark    
% \wei{refer to the figures in paper}
}\label{fig:data-summaries}
\end{figure*}

==> tab_tex/compare_img_diff_dataset.tex <==
\begin{table*} %[!tb]
    \centering
    \scriptsize
    \begin{tabular}{ccccM{1cm}M{1.5cm}ccccccc}
    \toprule
    Dataset &  image source & \# images & pairing & \# annotations & content &  average length & annotator & meta info   \\ 
    \midrule
    Spot-the-diff~\cite{spotthediff} & VIRAT video surveillance & 26k & video frame & 13k & difference description & & human   \\
    Scene Difference~\cite{li2023mimic} & COCO & 118k & image similarity &  142k  & & &  ChatGPT\\ 
    Comm diff  & Localized Narratives & 546k & overlapping nouns & 273k & commonality and difference & &Mixtral & CLIP sim, taxonomy \\
    \bottomrule
    \end{tabular}
    \caption{\wei{This table is to be removed} \wei{table layout and numbers need to be updated} Compare image diff dataset . We have other meta data  e.g. CLIP similarity score, taxonomy}
    \label{tab:my_label}
\end{table*}

==> tab_tex/compare_train_on_sgd_sd.tex <==
\begin{table*} %[!tb]
    \centering
    \scriptsize
    \begin{tabular}{ccccccccccccc}
    \toprule
    Training data &  BISON & SVO probes & EQBEN & COLA & NLVR2 &  VG Pair QA & VG Comm & VG diff  \\ 
    \midrule
    LLaVA data & 54.00 &  46.80 & 17.50 & 7.62 & 61.33 & 0.356 / 2.538  & 0.031 / 1.793 & 0.031 / 1.751 \\
    LLaVA + SD + Spot-the-diff & 84.67 & 87.80 & 20.83 & 26.67 & 62.67  & 0.469 / 2.920 & 0.050 / 1.188 & 0.392 / 2.900 \\ 
    LLaVA + Ours & 92.00 & 92.27 & 34.17 & 36.67 & 66.67 & 0.551 / 3.265 & 0.138 / 2.313 &  0.694 / 3.848  \\
    \bottomrule
    \end{tabular}
    \caption{\wei{This table is to be removed} Comparison to training on Scene Difference and Spot the diff (both are contained in the MIMIC-IT dataset)}
    \label{tab:my_label}
\end{table*}

==> tab_tex/eval_seed_bench.tex <==
\begin{table*} [!tb]
    \centering
    % \scriptsize
    \begin{tabular}{cccccccccc}
    \toprule
    Model &  LLaVA 1.5 7B & \OurMethod 7B & LLaVA 1.5 13B & \OurMethod 13B \\
    
    % xx & 1 & 2 \\
    % random chance & 25\% & 25\% & 25\% &50\% & 50\% & 50\% & 25\% & 25\% \\
    \midrule

        
        SEED-Image & 67.34\% & 67.48\% & 68.83\% & 69.11\%  \\

    \bottomrule
    \end{tabular}
    \caption{ Performance of multi-choice questions on SEED-Bench image partitions for evaluation of general VL capabilities with single-image input.}
    \label{tab:eval_seed_img}
\end{table*}

==> tab_tex/eval_seed_video.tex <==
\begin{table*} [!tb]
    \centering
    % \scriptsize
    \begin{tabular}{cccM{1cm}M{1cm}M{0.7cm}M{0.7cm}M{0.7cm}M{0.7cm}cccc}
    \toprule
    % Dataset &  SEED-V & SEED-V \\
    \# input frames & 1 & 2 \\
    % random chance & 25\% & 25\% & 25\% &50\% & 50\% & 50\% & 25\% & 25\% \\
    \midrule

        
        SparklesChat & 21.81\% &  19.09\%  ($\blacktriangledown$-2.72\%) \\
        Otter & 18.19\% & 23.00\% ($\blacktriangle$\textbf{+4.81\%}) \\
        % MMICL \wei{remove?} & 46.29\%  & 48.78\%\\
        EMU2-Chat  & \textbf{43.43\%} &  41.09\% ($\blacktriangledown$-2.34\%)  \\
        InternLM-XComposer2-VL 7B  & 41.07\% & 40.16\% ($\blacktriangledown$-0.91\%)\\
        LLaVA 1.6 7B  & \underline{41.95\%} & \underline{42.03\%} ($\blacktriangle$+0.08\%)  \\
        LLaVA 1.6 13B  & 41.85\% & 41.35\% ($\blacktriangledown$-0.50\%)  \\
        % Idefics2 & 43.39\%  &  44.95\% ($\blacktriangle$+1.56\%) \\
        \midrule
        LLaVA 1.5 7B   & 37.43\% & 36.68\% ($\blacktriangledown$-0.75\%) \\
        LLaVA 1.5 13B  & 40.12\% & 38.78\% ($\blacktriangledown$-1.34\%) \\
        \midrule
        \OurMethod 7B & 38.40\% & 40.44\% ($\blacktriangle$+2.04\%)  \\
        \OurMethod 13B  & 40.16\% & \textbf{43.09\%} ($\blacktriangle$\underline{+2.93\%}) \\
    \bottomrule
    \end{tabular}
    \caption{ Performance of multi-choice questions on SEED-Bench video partitions by feeding one or two frames into the LMMs. \wei{put this side-by-side with Table 4}}
    \label{tab:eval_seed_vid}
\end{table*}

==> tex/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes See Section~\ref{sec:conclusions}.
  \item Did you discuss any potential negative societal impacts of your work?
     \answerYes See Section~\ref{sec:conclusions}.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes 
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes In the supplementary. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes In Section~\ref{sec:results} and in supplementary.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes In the supplementary. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes In Section~\ref{sec:results} and in supplementary.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes We cite the papers of the original image and caption sources and the papers whose implementation we build upon. 
  \item Did you mention the license of the assets?
    \answerYes In the supplementary.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes our image sources are obtained from public datasets converted to \CaD VI data by our approach, we are releasing our data in accordance to the source data licenses.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes our image sources are obtained from public datasets converted to \CaD VI data by our approach, we are releasing our data in accordance to the source data licenses.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tex/phase2_method_description_old.tex <==
\myparagraph{LMM-based Instruction Data Collection.}
While in our phase 1 data collection we used an LLM to extract a \CaD summary based on human-generated captions, for phase 2 data collection we leverage our phase 1 model \OurModelPhaseOne and additional image pairs from various sources to extract the \CaD summaries informed by the images directly. The image sources for phase 2 can include: (i) existing difference-annotated datasets of similar image pairs Scene-Difference~\cite{li2023mimic} and Spot-the-diff \cite{spotthediff}; (ii) unlabeled pairs of video frames from Action Genome~\cite{ji2020action} and GEBC~\cite{wang2022geb+} (A/G). Scene-Difference~\cite{li2023mimic} contains pairs of similar images from COCO~\cite{lin2014microsoft} annotated with unstructured difference-only summaries (see Fig.~\ref{fig:pipeline} bottom left for an example). Spot-the-diff \cite{spotthediff} contains video frames of surveillance footage with human-annotated change description. 

When difference data is available (for image pairs from \cite{li2023mimic} and \cite{spotthediff}), we use it as part of the prompt to our \OurModelPhaseOne and completely re-annotate the image pair with the \CaD summary. As shown in  Fig.~\ref{fig:pipeline} (bottom row), our re-annotation leads to a more structured summary with both commonalities and differences. As part of our analysis, we show that in all cases our re-annotated data is significantly more effective for improving model's \CaD capabilities (Tab. \ref{tab:train_on_scene_diff} and \ref{tab:train_on_spot_the_diff}). Moreover, we also show that collecting data by annotating unlabeled frame pairs in A/G from scratch is significantly more effective than using the dataset-provided captions as prior information (Tab. \ref{tab:train_on_eqben}).   \wei{to re-structure,  also mention that Spot-the-diff is OOD data? }

In our phase 2 we collect 71K additional image pairs from Scene-Difference to form the \OurDataPhaseTwo dataset.   \wei{mention the number of pairs in each case}

% In order to further expand the knowledge of visual commonalities and differences, we leverage our phase-1 model \OurModelPhaseOne to annotate an existing image pair collection - Scene-Difference~\cite{li2023mimic} which contains 71K pairs of similar images from COCO~\cite{lin2014microsoft}. Scene-Difference provides annotation of difference descriptions for the image pairs. We feed both the image pairs and the original annotations into \OurModelPhaseOne, and generate the summary of commonalities and differences. This leads to our phase-2 CaD instruction data - \OurDataPhaseTwo.

% \wei{In order to demonstrate the \CaD annotation capability of \OurModelPhaseOne, we use \OurModelPhaseOne to annotate different types of images such as frames in user videos or surveillance footage, with different original annotations such as image caption or human-annotated difference description. We ablate on the image types and original annotation types in ee Sec.xxx }. we show that for either human-generated or LLM-generated \CaD sources, we can always significantly improve their data quality via our phase 2 targetted refinement by querying our phase 1 \OurModelPhaseOne model. 

\myparagraph{Phase-2 CaD Visual Instruction Tuning}
We follow the pipeline introduced in Sec.~\ref{sec:visual_instruct_tune} for CaD visual instruction tuning. Here we finetune on a combination of LLaVA 1.5 \cite{llava1_5} finetune data (665K), \OurDataPhaseOne data (278K) and \OurDataPhaseTwo data (71K). This phase of \CaD visual instruction tuning leads to the Stage-2 model, denoted as \OurModelPhaseTwo. 

==> tex/vlm_based_instruction_data_collection.tex <==
\section{Two-Stage Comparison Visual Instruction Tuning}

% \wei{TODO}
% \wei{Introduce concept of multi-phase? }
With our LLM-based instruction-following data collection - \OurDataPhaseOne, we perform visual instruction tuning on a Large Multimodal Model (LMM) LLaVA 1.5~\cite{llava1_5}, resulting in our cold-start Stage-1 model. In order to further expand the knowledge of visual commonalities and differences, we use the Stage-1 model to annotate an existing image pair collection - Scene-Difference~\cite{li2023mimic} which contains 71K pairs of similar images from COCO~\cite{lin2014microsoft}. We combine the data of \OurData and our annotated Scene-Difference for visual instruction tuning, leading to the Stage-2 model, denoted as \OurMethod (\textbf{Comp}arison visual instruction tuned \textbf{LLaVA}). We first 



\subsection{Re-annotation of Existing Datasets}\label{sec:}

train with LLM-annotated comm diff summary - the first-stage model with comparison capability 

use the first-stage model to re-annotate Scene-Difference data (70K), and train on Localized narratives + Scene difference data \wei{ablation - to show the quality of our re-annotation, refer to comparison between 1) llava + scene-diff original annot 2) llava + scene-diff our annot, Table~\ref{tab:train_on_scene_diff} }

\wei{ ablation of re-annotating Spot-the-diff (pair of video frames from satellite surveillance footage) and training on the re-annotated data - Table~\ref{tab:train_on_spot_the_diff} } \wei{Spot-the-diff dataset:  we select samples with images that are not included in SEED-Bench2} \wei{to show the quality of our re-annotation, refer to comparison between 1) llava + spot-the-diff original annot 2) llava + spot-the-diff our annot (in the spot-the-diff instruction-response data, we do not include the text-to-image retrieval task) }

\wei{ablation re-annotating  pairs of video frames from instruction videos in AG and GEBC, we use frame captions from EQBEN,  comparison result in Table~\ref{tab:train_on_eqben} }

% phase 3: use the phase 2 trained VLM to re-annotate Spot-the-diff (pair of video frames from satellite surveillance footage) and EQ-AG and EQ-GEBC (pair of video frames from instructional videos)







% \wei{uncurated pairs of images from localized narratives} \\
